Adapting SQuaRE for Quality Assessment of Artificial Intelligence Systems

More and more software practitioners are tackling towards industrial applications of artificial intelligence (AI) systems, especially those based on machine learning (ML). However, many of existing principles and approaches to traditional systems do not work effectively for the system behavior obtained by training not by logical design. In addition, unique kinds of requirements are emerging such as fairness and explainability. To provide clear guidance to understand and tackle these difficulties, we present an analysis on what quality concepts we should evaluate for AI systems. We base our discussion on ISO/IEC 25000 series, known as SQuaRE, and identify how it should be adapted for the unique nature of ML and $\textit{Ethics guidelines for trustworthy AI}$ from European Commission. We thus provide holistic insights for quality of AI systems by incorporating the ML nature and AI ethics to the traditional software quality concepts.

==> corner_case_measure.tex <==
\begin{table*}[ht]
\centering
\caption{SQuARE measures including corner cases}
\label{tab:corner_case_qme}
\begin{tabular}{@{} P{1.5cm}P{2cm}P{2.5cm}P{2.5cm}p{7.5cm} @{}} \toprule
\begin{tabular}{c}Quality\\model\end{tabular} & \begin{tabular}{c}Quality\\characteristic\end{tabular} & \begin{tabular}{c}Quality\\sub-characteristic\end{tabular} & \begin{tabular}{c}Quality\\measure\end{tabular} & \begin{tabular}{P{8.5cm}}QME\end{tabular} \\ \midrule
\multirow{18}{*}{\begin{tabular}{c}Product\\quality\end{tabular}} & \multirow{16}{*}{\begin{tabular}{c}Reliability\end{tabular}} & \multirow{6}{*}{\begin{tabular}{c}Maturity\end{tabular}} & \multirow{3}{*}{\begin{tabular}{c}Fault\\correction\end{tabular}} & Number of reliability-related {\bf faults} corrected in design/coding/testing phase \\ & & & & Number of reliability-related {\bf faults} detected in design/coding/testing phase \\ \cmidrule{4-5}
 & & & \begin{tabular}{c}Mean time\\between failure\end{tabular} & Number of system/software {\bf failures} actually occurred \\ \cmidrule{4-5}
 & & & Failure rate & Number of {\bf failures} detected during observation time \\ \cmidrule{3-5}
 & & Availability & \begin{tabular}{c}Mean\\down time\end{tabular} & Number of {\bf breakdowns} observed \\ \cmidrule{3-5}
 & & \multirow{6}{*}{\begin{tabular}{c}Fault tolerance\end{tabular}} & \multirow{4}{*}{\begin{tabular}{c}Failure\\avoidance\end{tabular}} & Number of avoided critical and serious {\bf failure} occurrences (based on test cases) \\ & & & & Number of executed test cases of fault pattern (almost causing {\bf failure}) during testing \\ \cmidrule{4-5}
 & & & \multirow{2}{*}{\begin{tabular}{c}Mean fault\\notification time\end{tabular}} & Time at which the {\bf fault} $i \dagger$ is reported by the system \\ & & & & Time at which {\bf fault} $i \dagger$ is detected \\ \cmidrule{3-5}
 & & \multirow{2}{*}{\begin{tabular}{c}Recoverability\end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}Mean\\recovery time\end{tabular}} & Total time to recover the downed software/system and re-initiate operation for each {\bf failure} $i \dagger$ \\ \cmidrule{2-5}
 & \multirow{2}{*}{\begin{tabular}{c}Maintainability\end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}Modifiability\end{tabular}} & \multirow{2}{*}{\begin{tabular}{c}Modification\\correctness\end{tabular}} & Number of modifications that caused an {\bf incident or failure} within a defined period after being implemented \\
\bottomrule 
\end{tabular}\\
\raggedleft
\begin{tabular}{c}\\$\dagger$ Summed or averaged over $i$\end{tabular}
\end{table*}


==> ethic_covered.tex <==
\begin{table*}[ht]
\centering
\caption{Ethical requirements covered by SQuARE}
\label{tab:ethic_req_cover}
\begin{tabular}{@{} P{2cm}P{2cm}p{6.25cm}p{6.25cm} @{}} \toprule
Requirement & Sub-requirement & \begin{tabular}{P{6.5cm}}Assessment Item\end{tabular} & \begin{tabular}{P{6.5cm}}SQuARE relationship\end{tabular} \\ \midrule
\multirow{2}{*}{\begin{tabular}{c}Human agency\\and oversight\end{tabular}} & \multirow{4}{*}{\begin{tabular}{c}Fundamental\\rights\end{tabular}} & Did you carry out a fundamental rights impact assessment where there could be a negative impact on fundamental rights? Did you identify and document potential trade-offs made between the different principles and rights? & EG4: SQuARE is system and software quality models and and will not cover fundamental rights. \\
 & \begin{tabular}{c}Fundamental\\rights\end{tabular} & Does the AI system interact with decisions by human (end) users (e.g. recommended actions or decisions to take, presenting of options)? &  \\
\bottomrule 
\end{tabular}
\end{table*}

